Restricted Discrete Invariance and Self-Synchronization For Stable Walking of Bipedal Robots

Models of bipedal locomotion are hybrid, with a continuous component often generated by a Lagrangian plus actuators, and a discrete component where leg transfer takes place. The discrete component typically consists of a locally embedded co-dimension one submanifold in the continuous state space of the robot, called the switching surface, and a reset map that provides a new initial condition when a solution of the continuous component intersects the switching surface. The aim of this paper is to identify a low-dimensional submanifold of the switching surface, which, when it can be rendered invariant by the closed-loop dynamics, leads to asymptotically stable periodic gaits. The paper begins this process by studying the well-known 3D Linear Inverted Pendulum (LIP) model, where analytical results are much easier to obtain. A key contribution here is the notion of \textit{self-synchronization}, which refers to the periods of the pendular motions in the sagittal and frontal planes tending to a common period. The notion of invariance resulting from the study of the 3D LIP model is then extended to a 9-DOF 3D biped. A numerical study is performed to illustrate that asymptotically stable walking may be obtained.

==> forward_ang_momentum.tex <==
\begin{tikzpicture}
\link (\thone:.75*\Lone);
\begin{scope}[shift=(\thone:.75*\Lone),rotate=0]
	\link (-\thone:.75*\Lone);
	\joint 
	\begin{scope}[shift=(-\thone:.75*\Lone),rotate=0]
		\node at (0,0) [below] {$O$};
		\link(\thone:.75*\Lone);
		\coordinate (mid) at ({.75*\Lone*cos(\thone)},0);
		\coordinate (midhalf) at ({.5*.75*\Lone*cos(\thone)},0);
                   \draw [dashed, black] (0,0)--(0,.75*\Lone);
                 %  \draw [->, very thick] (0,0) -- (mid);
                   \begin{scope}[shift=(90:.75*\Lone),rotate=0]
                   \end{scope}
		\begin{scope}[shift=(\thone:.75*\Lone),rotate=0]
			\link (-\thone:.75*\Lone);
			\joint
			\draw [dashed, black] (0,0) arc (\ArcAngle:\ArcAngle+2*(90-\thone):.75*\ArcRadius);	
			%\draw [dashed, black] (0,0) -- (mid);
			\begin{scope}[shift=(-\thone:.75*\Lone),rotate=0]
				\coordinate (minus_midhalf) at ({-.5*.75*\Lone*cos(\thone)},0);
				\robotbasethree
			\end{scope}
		\end{scope}
	\end{scope}
\end{scope}
\end{tikzpicture}


